Extracting or Guessing? Improving Faithfulness of Event Temporal Relation Extraction

In this paper, we seek to improve the faithfulness of TempRel extraction models from two perspectives. The first perspective is to extract genuinely based on contextual description. To achieve this, we propose to conduct counterfactual analysis to attenuate the effects of two significant types of training biases: the event trigger bias and the frequent label bias. We also add tense information into event representations to explicitly place an emphasis on the contextual description. The second perspective is to provide proper uncertainty estimation and abstain from extraction when no relation is described in the text. By parameterization of Dirichlet Prior over the model-predicted categorical distribution, we improve the model estimates of the correctness likelihood and make TempRel predictions more selective. We also employ temperature scaling to recalibrate the model confidence measure after bias mitigation. Through experimental analysis on MATRES, MATRES-DS, and TDDiscourse, we demonstrate that our model extracts TempRel and timelines more faithfully compared to SOTA methods, especially under distribution shifts.

==> ignore.tex <==
The idea of verb event tense marker comes from \cite{ZC21}.


Event temporal relation extraction baselines:
\begin{itemize}
    \item TemProb \cite{ning-etal-2018-improving}
    \item CogCompTime2.0 \cite{ning-etal-2019-improved}
    \item HMHD20 \cite{wang-etal-2020-joint}
    \item ZHN21 \cite{qiang-naacl-2022}
    \item hyperbolic \cite{tan-etal-2021-extracting}: 80.5 $F_1$
    \item Distant supervision \cite{zhao-etal-2021-effective} 79.6 $F_1$
    \item SMTL \cite{ballesteros-etal-2020-severing} 81.6 $F_1$; Data augmentaion (create a silver dataset as auxiliary task and then fine-tune using gold data) very insightful; better representation: $S_i, i = 1, \cdots, 5$
    \item TIMERS \cite{mathur-etal-2021-timers} 82.3 $F_1$
    \item selecting context sentences AAAI22 can be ignored \cite{trong2022selecting} 83.4 $F_1$ no code released
\end{itemize}




Spurious correlation, Debiasing, and Robustness:
\begin{itemize}
    \item Identifying and Mitigating Spurious Correlations for Improving Robustness in NLP Models \url{https://arxiv.org/pdf/2110.07736.pdf}
    \item Automatically Generating Counterfactuals for Relation Exaction \url{https://arxiv.org/abs/2202.10668}
    \item Should We Rely on Entity Mentions for Relation Extraction? Debiasing Relation Extraction with Counterfactual Analysis \url{https://openreview.net/pdf?id=9D65hK833L}
    \item Just Train Twice \cite{pmlr-v139-liu21f}
    \item Learning from Noisy Labels \cite{zhou-chen-2021-learning}
    \item Deep Ensemble \cite{NIPS2017_9ef2ed4b}
    \item Prior Networks \cite{malinin2018} KL Divergence
    \item Stephen Mayhew \cite{mayhew-etal-2019-named}
    \item Noisy-Labeled NER \cite{liu-etal-2021-noisy-labeled} 
    
    


    
\end{itemize}


Data for evaluation:
\begin{itemize}
    \item MATRES \cite{ning-etal-2018-multi}
    \item Contrast set \cite{gardner-etal-2020-evaluating}
    
\end{itemize}
